DocGenome: An Open Large-scale Scientific Document Benchmark for Training and Testing Multi-modal Large Language Models

Scientific documents record research findings and valuable human knowledge, comprising a vast corpus of high-quality data. Leveraging multi-modality data extracted from these documents and assessing large models' abilities to handle scientific document-oriented tasks is therefore meaningful. Despite promising advancements, large models still perform poorly on multi-page scientific document extraction and understanding tasks, and their capacity to process within-document data formats such as charts and equations remains under-explored. To address these issues, we present DocGenome, a structured document benchmark constructed by annotating 500K scientific documents from 153 disciplines in the arXiv open-access community, using our custom auto-labeling pipeline. DocGenome features four key characteristics: 1) Completeness: It is the first dataset to structure data from all modalities including 13 layout attributes along with their LaTeX source codes. 2) Logicality: It provides 6 logical relationships between different entities within each scientific document. 3) Diversity: It covers various document-oriented tasks, including document classification, visual grounding, document layout detection, document transformation, open-ended single-page QA and multi-page QA. 4) Correctness: It undergoes rigorous quality control checks conducted by a specialized team. We conduct extensive experiments to demonstrate the advantages of DocGenome and objectively evaluate the performance of large models on our benchmark.

==> sections/ethic.tex <==
\vspace{-6pt}
\section{Ethics Statement}
\vspace{-6pt}


==> tables/compared_language.tex <==

\begin{wrapfigure}{r}{0.49\textwidth}
\vspace{-4pt}
\begin{minipage}[t]{1\linewidth}
    \centering
\captionof{table}{QA results using different LLMs.}
\resizebox{1\textwidth}{!}
{
\setlength{\tabcolsep}{1.6mm}{
\begin{tabular}{cccc}
\hline
\multirow{2}{*}{Models} & \multirow{2}{*}{Vision Encoder}  & \multirow{2}{*}{Language Decoder} & QA Results \\
    &  &  & GPT-acc \\ 
\hline
StructTable-B  & ViT-0.3B & LlaMA-7B &  - \\
StructTable-B & ViT-0.3B & LlaMA-13B & - \\ 
StructTable-B & ViT-0.3B & Vicuna-7B & - \\ 
StructTable-B & ViT-0.3B & Vicuna-13B & - \\ 
\hline
\end{tabular}}
}
\label{tab:ablation}
%\end{table}
\end{minipage}
\end{wrapfigure}

==> tables/compared_sota_table.tex <==

\begin{table*}[t]
\vspace{-0.60cm}
    \small
	\centering	
    \setlength\tabcolsep{4pt}
    \caption
	{
	\small	
        Comparison with state-of-the-art multi-modal language models on our proposed TableX, including table image-to-tex, table captioning, and table QA tasks. The employed evaluation metric for each task can be found in Sec.~\ref{}.
	}
	\resizebox{1\textwidth}{!}{
	\begin{tabular}	{l l |  c  c  c | c | c   }
	\toprule	 	
	 \multirow{3}{*}{Model} & \multirow{3}{*}{{\#Params}} &\multicolumn{5}{c}{Table-related Tasks}  \\
	 & &    \multicolumn{3}{c}{Table-to-Tex}& \multicolumn{1}{c}{Table Captioning} & \multicolumn{1}{c}{Table QA} \\
	     
	& &  ROUGE-1 & ROUGE-2 & BLEU & Acc & GPT-acc   \\
	\midrule  
    \textit{~~Multi-modal Large Models} \\
        LlaVA-1.5~\cite{liu2023improved} & 13B &
	0.04 & 0.04 & 0.24 & 47.05 & 44.18 
	\\
        CogVLM~\cite{wang2023cogvlm} & - 
	&   &   &   &   &   
	\\    
        QWen-VL~\cite{bai2023qwen} & -
	&   &   &   &   &   
	\\    
        SPHINX-V2~\cite{lin2023sphinx} & -
	&   &   &   &   &  
	\\
	GPT-4V~\cite{yang2023dawn}& - 
	&   &   &   &   &  
	\\
	\midrule
    
	\multicolumn{2}{l}{\textit{~~Ours}} \\ 
    \textbf{TableVLM-B} & 7.3B 
    &   &   &   &   &   
    \\
    \bottomrule
	\end{tabular}
	}
	\label{tab:compared_sota}
\end{table*}	

==> tables/equation.tex <==
\begin{table*}[!t]
    % \aboverulesep = 0.48mm
    % \belowrulesep = 0.48mm
    \small
	\centering	
    \setlength\tabcolsep{4pt}
    \caption
    {
	\small	
        Results using different amounts of table data, show the scalable model capacity for tackling the table-related tasks. The employed evaluation metric for each task can be found in Sec.~\ref{}.
	}
	\resizebox{1\textwidth}{!}{
	\begin{tabular}	{l l |  c  c  c  c }
	\toprule	 	
	 \multirow{2}{*}{Model} &\multirow{2}{*}{{\#Data Amount}} &\multicolumn{4}{c}{Equation-to-Tex}  \\
    %\cline{3-6}
	 & & Edit Distance$\downarrow$ & Jaccard Similarity$\uparrow$ & Cosine Similarity$\uparrow$& BLEU$\uparrow$  \\
	\midrule  
    \multicolumn{2}{l}{\textit{~~DocGenome-test}} \\ 
	Mathpix& N/A 
	& 78.25  & 0.7226  & 0.6045  & 0.4472  
	\\
    EqVLM-B & 10k
    & 74.89 & 0.8157  & 0.7840  & 0.5165 
    \\
    EqVLM-B & 100k
    & 52.99  & 0.8505  & 0.8317  & 0.5862
    \\
    \textbf{EqVLM-B} & 1M
    &  40.23 &  0.8736 & 0.8621  &  0.6352
    \\

	\midrule

    \multicolumn{2}{l}{\textit{~~SCI-Hub}} \\ 
    Mathpix& N/A 
	& \textcolor{red}{356.2}  & 0.7437  & 0.7295  & 0.1137  
	\\
    EqVLM-B& 10k
    &  489.7 & 0.6164  & 0.5712  & 0.0536 
    \\
    EqVLM-B& 100k
    & 460.3  & 0.6303  & 0.5726  & 0.0602 
    \\
    \textbf{EqVLM-B}& 1M
    &  470.1 &  0.6234 &  0.5346 &  0.0671 
    \\
    \bottomrule
	\end{tabular}
	}
	\label{tab:equation}
\vspace{-4pt}
\end{table*}	


==> tables/layout_detection.tex <==

\begin{table*}[!t]
    % \aboverulesep = 0.48mm
    % \belowrulesep = 0.48mm
    \small
	\centering	
    \setlength\tabcolsep{4pt}
    \caption
	{
	\small	
        Comparison of state-of-the-art layout detection models on our proposed test-DocGenome, using AP@0.5-0.95 metric to evaluate the results.
	}
	\resizebox{1\textwidth}{!}{
	\begin{tabular}	{c |  c  | c  | c  c  c c c c c }
	\toprule	 	
        Model & Data Amount & mAP@0.5-0.95$\uparrow$  &  Title & Text & Figure   & Caption  & Equation  &  Table &  Footnote\\
	\midrule  
    \multicolumn{2}{l}{\textit{~~Auto-labeled Evaluation Set}} \\ 
        DocXChain~\cite{yao2023docxchain} & N/A &53.20
	& 49.21 & 79.22 & 43.85  & 48.18 & 49.36 & 72.79 & 29.79
	\\
         YOLOv8~\cite{yolov8} & 7k & 77.47
	&  71.79 & 92.48 & 76.29 & 86.56 & 80.65 & 85.81  & 48.43
    \\
            YOLOv8~\cite{yolov8} & 70k & 89.42
	&  83.46 & 95.56 & 86.36 & 94.92 & 90.13 & 92.77  & 82.72
    \\
        YOLOv8~\cite{yolov8} & 700k &91.37
	&  86.05 & 95.96 & 88.46 & 95.71 & 93.06 & 93.77  & 86.52
    \\
	\midrule  
    \multicolumn{2}{l}{\textit{~~Human-labeled Evaluation Set}} \\ 
        DocXChain~\cite{yao2023docxchain} & N/A & 37.99
	& 32.53 & 59.00 & 67.17 & 38.71  & 12.98 & 38.99 & 16.54
	\\
        YOLOv8~\cite{yolov8} & 700k & 50.15 
	& 42.59  &  64.87   & 56.65 & 64.51 & 47.14 & 47.08  & 28.21
    \\
    \bottomrule
	\end{tabular}
	}
	\label{doc:layout_detection}
\vspace{-4pt}
\end{table*}	

==> tables/table_scale_up_new.tex <==
\begin{table*}[t]
    \small
	\centering	
    \setlength\tabcolsep{4pt}
    \caption
    {
	\small	
        Results on scaling up the data using the DocGenome-train, showing the scalable model capacity for tackling the table transformation task. TableVLM-B means that we train a visual encoder and a text decoder using the DocGenome-train for the table transformation task. See Sec.~\ref{} for the employed metric.
	}
    \vspace{-0.25cm}
	\resizebox{0.90\textwidth}{!}{
	\begin{tabular}	{l l |  c  c  c  c }
	\toprule	 	
	 \multirow{2}{*}{Model} & \multirow{2}{*}{{ Training Data Amount}} &\multicolumn{4}{c}{Table-to-LaTex}  \\
    %\cline{3-6}
	 & &  Edit Distance$\downarrow$ & Jaccard Similarity$\uparrow$ & Cosine Similarity$\uparrow$& BLEU$\uparrow$  \\
	\midrule  
	Mathpix\tablefootnote[4]{Online API we used for evaluation: \textcolor{teal}{\url{https://mathpix.com/table-to-latex}}}  & N/A 
	& 434.7  & 0.7730  & 0.5826  & 0.3528  
	\\
	\midrule
    
	\multicolumn{2}{l}{\textit{~~Ours}} \\ 
    TableVLM-B & 5K
    & 535.9  & 0.8185  & 0.7804  & 0.4596 
    \\
    TableVLM-B & 10K
    & 513.8  & 0.8635  & 0.8187  & 0.4973  
    \\
    TableVLM-B & 100K
    & 356.4  & 0.8903  & 0.8571  & 0.5340   
    \\
    \textbf{TableVLM-B} & 500K
    & \textbf{297.7}  & \textbf{0.8997}  & \textbf{0.8800}  & \textbf{0.5552}  
    \\
    % \textbf{TableVLM-B} & 1M
    % &   &   &   &   &   
    % \\
    \bottomrule
	\end{tabular}
	}
\label{tab:table_scaleup}
\vspace{-4pt}
\end{table*}	
